FpgaHub: Fpga-centric Hyper-heterogeneous Computing Platform for Big Data Analytics

Modern data analytics requires a huge amount of computing power and processes a massive amount of data. At the same time, the underlying computing platform is becoming much more heterogeneous on both hardware and software. Even though specialized hardware, e.g., FPGA- or GPU- or TPU-based systems, often achieves better performance than a CPU-only system due to the slowing of Moore's law, such systems are limited in what they can do. For example, GPU-only approaches suffer from severe IO limitations. To truly exploit the potential of hardware heterogeneity, we present FpgaHub, an FPGA-centric hyper-heterogeneous computing platform for big data analytics. The key idea of FpgaHub is to use reconfigurable computing to implement a versatile hub complementing other processors (CPUs, GPUs, DPUs, programmable switches, computational storage, etc.). Using an FPGA as the basis, we can take advantage of its highly reconfigurable nature and rich IO interfaces such as PCIe, networking, and on-board memory, to place it at the center of the architecture and use it as a data and control plane for data movement, scheduling, pre-processing, etc. FpgaHub enables architectural flexibility to allow exploring the rich design space of heterogeneous computing platforms.

==> content/background.tex <==
\section{Background}
\label{sec_background}
%\vspace{-1ex}
In this section, we briefly discuss the necessary background, including GPUDirect, FPGA, and SmartNIC. 
\vspace{-1ex}
\subsection{NVIDIA GPUDirect Technology}
\vspace{-1ex}
NVIDIA GPUDirect technology enables direct PCIe P2P data communication between a GPU and a third-party PCIe device, e.g., Mellanox ConnectX-5 NIC~\cite{mellanox-bluefield}. Such a technology is able to eliminate additional staging at the host memory, significantly lowering CPU overhead and thus improving data transfer efficiency.\footnote{AMD also provides the DirectGMA technique~\cite{directgma} for its GPUs.}% or Xilinx U280 FPGA board~\cite{u280}

% \vspace{-1ex}
% \subsubsection{GPUDirect RDMA}% (Data Plane Offload)
% \vspace{-1ex}
\noindent{\bf GPUDirect RDMA. }GPUDirect RDMA~\cite{gpudirect_rdma} is a technology that enables a third-party PCIe peer device like Mellanox's NIC to directly initiate an RDMA operation to read from or write to GPU memory, which is exposed to the third-part PCIe device via a GPU Base Address Registers (BAR) window, whose size varies with GPU class. For example, the Quadro-class GPU RTX 8000 that features a 32-bit BAR register only allows 220MB BAR size,\footnote{The available BAR size is 256MB, the remaining 32MB is reserved for internal use~\cite{gpudirect_rdma}.} while the Tesla-class GPU V100 with a 64-bit BAR register exposes at least 31GB BAR size to a PCIe peer device. %GPU BAR mapping 

%Phicial address, virtual address.. GPU page size is 64KB. 
% \vspace{-1ex}
% \subsubsection{GPUDirect Async} % (Control Plane Offload)
% \vspace{-1ex}
% GPUDirect Async~\cite{gpudirect_rdma} is a technology that allows offloading control plane onto the GPU, such that the GPU is able to directly trigger communication operations without CPU intervention. To achieve this, the CUDA driver provides a memory management function \emph{cudaHostRegister}, which registers an existing host address of a contiguous range for use by within a CUDA kernel, and provides the \emph{cudaHostRegisterIoMemory} flag that allows the host address to map to an MMIO address of a third-part PCIe device like Mellanox HCA~\cite{connectx5}.\footnote{In this paper, we enable an FPGA to be a third-part PCIe device directly accessed by the GPU.} However, the use of GPUDirect Async has to combine with a PCIe P2P-aware NIC that provides necessary doorbell registers and the corresponding driver complementary to GPUDirect Async. Therefore, combining GPUDirect Async, Mellanox Infiniband NIC, and Mellanox OFED (OpenFabrics Enterprise Distribution)~\cite{ofed} to enable the GPU directly trigger communication operation on the Infiniband NIC. %Therefore, GPUDirect Async itself cannot directly manipulate a third-part PCIe device like Mellanox Infiniband NIC. 

% \vspace{-1ex}
% \subsection{PCIe-based FPGA Acceleration Board}
% \label{sub_pcie_fpga_card}
% \vspace{-1ex}
% Recently, FPGA vendors provide off-the-shelf FPGA acceleration cards~\cite{xilinx_alveo, intel_stratix} such as Xilinx's Alveo cards, which aim to accelerate compute tasks offloaded from the host CPU. These FPGA cards typically feature a PCIe interface for communicating with the host and network interface(s) for communicating with other network devices. In this paper, we intend to transform these FPGA boards into SmartNICs, capable of cooperating with GPUs to optimize the efficiency of the whole system. %Besides, FPGA programmers are capable of doing SmartNIC-related research and deployment with off-the-shelf FPGA acceleration boards at their disposal. %without the need to buy a dedicated SmartNIC.  
 
% The main component of the board is an FPGA, consisting of lookup tables (LUTs), registers (REGs), on-chip block rams (BRAMs), on-chip DSPs. The FPGA can be used to implement specialized pipelined digital circuits for a given application, offering higher energy efficiency and better performance guarantees than running the application on CPUs/GPUs. However, we originally program FPGAs with Hardware Description Languages (HDL), which is well-known to be difficult to program and then hinders FPGAs from wide adoption by software programmers. Fortunately, FPGA vendors such as Xilinx started to provide High Level Synthesis (HLS)~\cite{xilinxhls, alteraopencl} for much higher programmability as a way to attract software programmers to accelerate their applications. 


%\vspace{-1ex}
\subsection{FPGA-augmented SmartNICs}
\label{sub_pcie_fpga_card}
%\vspace{-1ex}
%\violet{Innvo is an FPGA-augmented SmartNIC that features an FPGA to connect to the network ASIC via the chip-to-chip interconnect PCIe. Figure...} 
Mellanox Innova-2 is An FPGA-augmented SmartNIC that features a network adapter ConnectX-5 and an Xilinx FPGA, as shown in Figure~\ref{P_innova} (a). ConnectX-5 consists of a 100Gbs InfiniBand/Ethernet interface for networking and a PCIe Gen4x8 interface for communicating with the host CPU. The FPGA, which communicates with ConectX-5 via a PCIe x8 Gen4 link, can be entirely dedicated its own resources to application logic. However, the limitation of Innova lies in its limited bandwidth between the FPGA and ConnectX-5. The FPGA can only consume data stream either from line-rate 100Gbps network or from line-rate 100Gbps PCIe, motivating the design of \sysname{} that removes this limitation by implementing the network adapter within an FPGA, as shown in Figure~\ref{P_innova} (b). 

\begin{figure}[t]
	\centering
	\includegraphics[width=7.6cm]{figure/innova.pdf}
	\vspace{-1ex}
	\caption{Architecture differences between Innova-2 and \sysname }
	\vspace{-2ex}
	\label{P_innova}
\end{figure}

%In this paper, we intend to transform these FPGA boards into FPGA-based SmartNICs, which are capable of cooperating with GPUs to improve total system performance. As such, the FPGA programmer is capable of doing SmartNIC-related research without the need to buy a dedicated FPGA-based SmartNIC like Innova. 



==> content/p4sgd_latency.tex <==
% -----------------------------------------------------------------------------
\begin{figure}[h]
\centering
  \begin{tikzpicture}
  
  \begin{axis}[
  	boxplot/draw direction=y,
    width=1\columnwidth,
	height=0.55\columnwidth,
    xtick={0, 2},
    xticklabels={\scriptsize{P4SGD}, \scriptsize{SwitchML}},%
    ylabel={Latency [$\mu s$]},
    ymin=0.0,
    ymajorgrids=true,

    legend style={at={(0.5,1.05)},
          anchor=south, font=\footnotesize},
    legend columns=2,
    legend cell align=left,
  ]
  \pgfplotstableread{data/p4sgd_latency.dat}\datatable
  \pgfplotsinvokeforeach{0} % P4SGD
  {
  	\addplot[
    	boxplot prepared from table={
      		table=\datatable, row=#1,
      		lower whisker=1p, upper whisker=99p, lower quartile=25p, upper quartile=75p, median=median, draw position=pos
        },
    	boxplot prepared={ box extend=0.5, },
    	fill=red!40,
    	postaction={pattern=crosshatch},
    	area legend
    ] coordinates {};
  }

  \pgfplotsinvokeforeach{1} % SwitchML
  {
  	\addplot[
    	boxplot prepared from table={
      		table=\datatable, row=#1,
      		lower whisker=1p, upper whisker=99p, lower quartile=25p, upper quartile=75p, median=median, draw position=pos
        },
    	boxplot prepared={ box extend=0.5, },
    	fill=blue!40,
    	postaction={pattern=north west lines},
    	area legend
    ] coordinates {};
  }
  
  \end{axis}
  \end{tikzpicture}
  \vspace{-1ex}
  \caption{Latency.}
  \vspace{-2ex}
  \label{fig:p4sgd_latency_box}
\end{figure}
% -----------------------------------------------------------------------------


==> content/relatedwork.tex <==
\section{Related Work}
\label{sec_relatedwork}
	\vspace{-1ex}
To our knowledge, \sysname{} is an FPGA-based GPU-centric 100Gbps SmartNIC allowing a large design space exploration. %FPGA-based SmartNIC that supports 100Gbps TCP stack and direct data communication with GPUs via PCIe 3.0 x16, while allowing the offloading of compute tasks. %memory-intensive and/or compute-intensive application-level kernels due to its HBMs and sufficient spare FPGA resources. %We contrast closely related work with \sysname{} on 1) benchmarking traditional memory on FPGAs; 2) data processing with HBM; and 3) accelerating application with FPGAs. %three aspects.  a full-stack FPGA-based SmartNIC that opens up the opportunity to explore a large design space around SmartNICs due to FPGA’s reconfiguable nature


\noindent{\bf FPGA-augumented SmartNICs. }Several commercial systems~\cite{intel_smartnic, innova_mellanox18, catapult1, catapult2, intel_ipu, zilberman2014netfpga} feature an FPGA within a SmartNIC. The closest work is from Mellanox Innova~\cite{innova_mellanox18} that features an FPGA in its SmartNIC to accelerate offloaded compute-intensive applications, while PCIe and network interfaces are handled by a NIC ASIC ConnectX-5. The FPGA is connected with the NIC ASIC via a PCIe interface and therefore acts as an additional PCIe endpoint. The FPGA is entirely dedicated to the user's application logic. In contrast, \sysname{} implements all functionalities, including networking and PCIe, within a powerful FPGA, enabling a large design space exploration of SmartNIC architecture, while Innova provides limited architectural flexibility due to how the FPGA is connected.%ADD MORE!!!%significantly more architectural freedom for programmers. , as shown in Figure~\ref{P_innova} (a)

%\noindent{\bf GPU-FPGA Communication. }Plenty of previous work \cite{FPGA2_fpga13, direct_GPU_FPGA_icppw12} has implemented GPUDirect RDMA on an FPGA to directly access GPU memory, but not allowing the GPU to trigger doorbell registers within an FPGA. In contrast, \sysname{} allows GPUDirect RDMA and the GPU to trigger registers within an FPGA, and is an FPGA-based SmartNIC that allows large design space exploration of SmartNIC architecture. 

%\noindent{\bf GPU-FPGA Communication. }Plenty of previous work~\cite{lynx_asplos201} . 

\noindent{\bf Acceleration using FPGA-based SmartNICs. }Most previous work \cite{li2017kvdirect, dagger_nic20, msr2018smartnic, nica_atc19, strom_eurosys20, li2017kvdirect, msr2018smartnic, catapult2, DUA_nsdi19, transport_nsdi20, scatter_gather_socc20, hxdp_osdi20, incondemand_eurosys19, clicknp_sigcomm16} features an FPGA on SmartNICs to offload data processing to the network from the host CPU. In contrast, \sysname{} is an FPGA-based full-stack SmartNIC that mainly targets compute task offloading from local GPUs which requires a more complex system than offloading for CPUs. % ~\cite{panic_osdi20, nica_atc19} Particularly, previous work~\cite{nica_atc19, innova_mellanox18} leverages an FPGA as a off-path accelerator on the SmartNIC for offloading compute-intensive tasks. serves its local GPUs,

\noindent{\bf Multicore-based SmartNICs. }There is also a lot of work done \cite{mellanox-bluefield, ipipe_sigcomm19, fairnic_sigcomm20, floem_osdi18, lynx_asplos20, alek2014farm, jumpgate_hotcloud19, e3_atc19, yournic_hotnets18, clara_hotnets20, flexnic_asplos16, learned_cache_osdi20, accelTCP_NSDI_20} on SmartNIC built upon a wimpy RISC cores plus hardware engines to accelerate dedicated functionality such as compression. These RISC cores are used to both process packets as well as to implement ``smart" functions instead of using the host CPUs. Such an approach inevitably suffers from load interference since packet processing and the smart functions have to compete for the shared resources, e.g., the last level cache and memory bandwidth. In contrast, \sysname{} is an FPGA-based GPU-centric SmartNIC.  %\textcolor{red}{NVIDIA's recent BlueField-2 card supports two high speed network interfaces and features a 8-core ARM processor which runs a customized version of Linux. However, the processor has trouble saturating the 100Gbps network link. It can only generate approximately 60\% of the total bandwidth \cite{bf2_benchmark} in separated host mode even using all threads and generating large packets. \sysname{} can guarantee performance because it provides dedicated hardware resources for each offloaded compute task.} %Project Monterey from VMware~\cite{vmware_menterey} introduces SmartNICs, e.g., NVIDIA BlueField-2, to redefine hybrid cloud architecture in its VMware Cloud Foundation. 

\noindent{\bf On-going SmartNICs in Industry. }
Besides NVIDIA's DPU, Broadcom presents its Stingray SmartNIC~\cite{broadcom}, which features a ARM 8-core CPU for control-plane management and P4-like TruFlow packet processing engine for data-plane processing. 
Pensando present its DPU architecture~\cite{pensando_dsc} that features an ARM CPU and a P4 processor for data-plane packet processing. Netronome presents its NFP4000 Flow Processor architecture~\cite{Netronome_nfp4k} that features a ARM CPU, 48 P4-programmable packet processing cores, and 60 P4-programmable flow processing cores for data-plane processing. Fungible present its DPU, whose actual architecture and makeup is unclear. Intel presents the FPGA-based IPU (Infrastructure Processing Unit) that consists of a MAX 10 FPGA for control-plane management and an Arria 10 FPGA for data-plane processing~\cite{intel_fpga_smartnic}, and presents the ASIC IPU whose architecture is unclear~\cite{intel_ipu_smartnic}. 
Fungible presents its DPU~\cite{fungible_dpu} that features PCIe, networking, and various computing engines to address inefficient data-centric computation within a node and inefficient interchange between nodes. In contrast, \sysname{} is an FPGA-based GPU-centric SmartNIC.




%to deliver high performance and zero-trust security. %that is able to guarantee performance of smart functionality by leveraging dedicated hardware resources and memory channels (e.g., HBM). %to implement. Add VMware's project Meteray
%Using multicore to  suffer from the interference 


